Exemplars-guided Empathetic Response Generation Controlled by the Elements of Human Communication

The majority of existing methods for empathetic response generation rely on the emotion of the context to generate empathetic responses. However, empathy is much more than generating responses with an appropriate emotion. It also often entails subtle expressions of understanding and personal resonance with the situation of the other interlocutor. Unfortunately, such qualities are difficult to quantify and the datasets lack the relevant annotations. To address this issue, in this paper we propose an approach that relies on exemplars to cue the generative model on fine stylistic properties that signal empathy to the interlocutor. To this end, we employ dense passage retrieval to extract relevant exemplary responses from the training set. Three elements of human communication -- emotional presence, interpretation, and exploration, and sentiment are additionally introduced using synthetic labels to guide the generation towards empathy. The human evaluation is also extended by these elements of human communication. We empirically show that these approaches yield significant improvements in empathetic response quality in terms of both automated and human-evaluated metrics. The implementation is available at https://github.com/declare-lab/exemplary-empathy.

==> case_studies.tex <==


















    ### DON'T USE ###


























\begin{table*}[ht!]
\small
\centering
\begingroup
\setlength{\tabcolsep}{6.5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\caption{Comparing responses between models.}
\label{tab:case_study}
\resizebox{0.95\linewidth}{!}
{\begin{tabular}{|l|l|ccccc|}
\hline
& & \textbf{Relevance} & \makecell{\textbf{Emotional}\\\textbf{Presence}} & \textbf{Interpretation} & \textbf{Exploration} & \textbf{Winner} \\
\hline

\textbf{Emotion} & \textsc{TERRIFIED} & & & & & \\
\textbf{Context} & \makecell[l]{My dad called me one day crying out for help. I had to drive \\ over to his house.} & & & & & \\
\textbf{Reference} & Oh my goodness! What happened? & & & & & \\
% \textbf{Exemplar} & Oh that's terrible. Is he okay? & & & & & \\
\cline{2-2}
\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}} & Oh no, did he get hurt? I hope it wasn't too bad. & \cellcolor{Green2} High & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Green2} High & \multirow{4}{*}{\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}}} \\
\makecell[r]{\colorbox{ghostwhite}{\textsc{T5-GloVe}}} & That's awful. Is he okay? Does it have someone you can do that & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \\
\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}} & That is good to hear. How did he die? & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Blue1}{\textsc{EmpDG}}} & That is so sweet. I am sure you are so hard. & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL &  \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\

\hline
\hline

\textbf{Emotion} & \textsc{CONFIDENT} & & & & & \\
\textbf{Context} & \makecell[l]{I know I shouldn't count my chicks before they hatch, \\ but I'm feeling pretty good after that interview today!} & & & & & \\
\textbf{Reference} & Oh what job was the interview for? & & & & & \\
% \textbf{Exemplar} & \makecell[l]{Awesome! My husband had an interview as well. I hope both of \\ our spouses get a job.} & & & & & \\
\cline{2-2}
\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}} & That is great. You must have felt proud of yourself! I am sure you will get it. & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \multirow{4}{*}{\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}}}\\
\makecell[r]{\colorbox{ghostwhite}{\textsc{T5-GloVe}}} & Oh wow. I bet the zoo is really amazing! You can do it! & \cellcolor{Gray1} NIL & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}} & I bet you are so proud of yourself! & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Blue1}{\textsc{EmpDG}}} & What kind of I do you think you will do? & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\

\hline
\hline

\textbf{Emotion} & \textsc{SENTIMENTAL} & & & & & \\
\textbf{Context} & \makecell[l]{I was heartbroken when my dad passed away.. still not over it.} & & & & & \\
\textbf{Reference} & \makecell[l]{Sorry to hear that... they say time heals everything but i disagree its \\ been 9 years for me and it still feels like yesterday. How long for you?} & & & & & \\
% \textbf{Exemplar} & \makecell[l]{I am so sorry to hear that.  Losing a loved one is definitely \\ one of the hardest things in life.} & & & & & \\
\cline{2-2}
\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}} & I'm sorry to hear that. It's so hard to lose a friend. & \cellcolor{Green2} High & \cellcolor{Green2} High & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \multirow{4}{*}{\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}}}\\
\makecell[r]{\colorbox{ghostwhite}{\textsc{T5-GloVe}}} & Oh that's terrible . What happened? Your aunt's wrong ? & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}} & Oh, I am sorry. I hope he was a good thing to do. &\cellcolor{Green0} Low & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Blue1}{\textsc{EmpDG}}} & I am so sorry to hear that. &\cellcolor{Green0} Low & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\

\hline
\hline

\textbf{Emotion} & \textsc{ANNOYED} & & & & & \\
\textbf{Context} & \makecell[l]{I left my food on the coffee table and my dog ate it.} & & & & & \\
\textbf{Reference} & That is a terrible tragedy, my friend. Did the dog get sick? & & & & & \\
% \textbf{Exemplar} & Was the dog okay? & & & & & \\
\cline{2-2}
\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}} & That sucks. You must have been angry. That happens to me. & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \multirow{4}{*}{\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}}}\\
\makecell[r]{\colorbox{ghostwhite}{\textsc{T5-GloVe}}} & Oh that' s terrible, I hope you can find a friend! &\cellcolor{Green0} Low & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}} & That sounds really frustrating. What happened? & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Blue1}{\textsc{EmpDG}}} & Oh no! What happened? & \cellcolor{Green1} Mid  & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\

\hline
\hline

\textbf{Emotion} & \textsc{CONFIDENT} & & & & & \\
\textbf{Context} & \makecell[l]{I felt pretty good leaving the gym today, hit a new PR on overhead press} & & & & & \\
\textbf{Reference} & That's great. You must have been working really hard. & & & & & \\
% \textbf{Exemplar} & It sounds like you were very prepared!! Good job! & & & & & \\
\cline{2-2}
\makecell[r]{\colorbox{brilliantlavender}{\textsc{ExEmpt}}} & Awesome, that is great! Did you have a good time? I love doing that. & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \multirow{5}{*}{\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}}}\\
\makecell[r]{\colorbox{ghostwhite}{\textsc{T5-GloVe}}} & \makecell[l]{That is awesome! You must be pretty proud! You should be pretty \\ proud of yourself.} & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Green1} Mid & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Yellow1}{\textsc{MIME}}} & I bet that is a lot of hard work. & \cellcolor{Green2} High & \cellcolor{Green1} Mid & \cellcolor{Green2} High & \cellcolor{Gray1} NIL & \\
\makecell[r]{\colorbox{Blue1}{\textsc{EmpDG}}} & Oh no! I am so sorry! I bet you were mad! & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \cellcolor{Gray1} NIL & \\

\bottomrule
\end{tabular}
}
\endgroup
\end{table*}

